MUSCLE: Multi-task Self-supervised Continual Learning to Pre-train Deep Models for X-ray Images of Multiple Body Parts

While self-supervised learning (SSL) algorithms have been widely used to pre-train deep models, few efforts [11] have been done to improve representation learning of X-ray image analysis with SSL pre-trained models. In this work, we study a novel self-supervised pre-training pipeline, namely Multi-task Self-super-vised Continual Learning (MUSCLE), for multiple medical imaging tasks, such as classification and segmentation, using X-ray images collected from multiple body parts, including heads, lungs, and bones. Specifically, MUSCLE aggregates X-rays collected from multiple body parts for MoCo-based representation learning, and adopts a well-designed continual learning (CL) procedure to further pre-train the backbone subject various X-ray analysis tasks jointly. Certain strategies for image pre-processing, learning schedules, and regularization have been used to solve data heterogeneity, overfitting, and catastrophic forgetting problems for multi-task/dataset learning in MUSCLE.We evaluate MUSCLE using 9 real-world X-ray datasets with various tasks, including pneumonia classification, skeletal abnormality classification, lung segmentation, and tuberculosis (TB) detection. Comparisons against other pre-trained models [7] confirm the proof-of-concept that self-supervised multi-task/dataset continual pre-training could boost the performance of X-ray image analysis.

==> dataset-v2.tex <==

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\vspace{-5mm}
\begin{table}\centering
\caption{An Overview of Nine Publicly Available X-ray Image Datasets.}
%\resizebox{.95\columnwidth}{!}{
\begin{tabular}{p{150 pt}p{50 pt}p{50 pt}p{50 pt}}
\hline
\multicolumn{1}{c}{\bfseries Datasets} & \multicolumn{1}{c}{\bfseries Body Part} & \multicolumn{1}{c}{\bfseries Task} & \multicolumn{1}{c}{\bfseries Dataset Size}\\
\hline
\multicolumn{4}{c}{Only Used for the first step (MD-MoCo) of \TheName{}}\\\hline
NIHCC~\cite{ref_article_15} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{N/A} & \multicolumn{1}{r}{112,120}\\
China-Set-CXR~\cite{ref_article_16} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{N/A} & \multicolumn{1}{r}{661}\\
Montgomery-Set-CXR~\cite{ref_article_16} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{N/A} & \multicolumn{1}{r}{138}\\
Indiana-CXR~\cite{ref_article_17} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{N/A} & \multicolumn{1}{r}{7,470}\\
RSNA Bone Age~\cite{ref_article_20} & \multicolumn{1}{c}{Hand} & \multicolumn{1}{r}{N/A} & \multicolumn{1}{r}{10,811}\\\hline
\multicolumn{4}{c}{Used for all three steps of \TheName{}}\\\hline
Pneumonia~\cite{ref_article_18} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{\tabincell{r}{CLS}} & \multicolumn{1}{r}{5,856}\\
MURA~\cite{ref_article_21} & \multicolumn{1}{c}{\tabincell{c}{Various Bones}} & \multicolumn{1}{r}{\tabincell{r}{CLS}} & \multicolumn{1}{r}{40,005}\\
Chest Xray Masks and Labels~\cite{ref_article_16} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{\tabincell{r}{SEG}} & \multicolumn{1}{r}{896}\\
TBX~\cite{ref_article_22} & \multicolumn{1}{c}{Chest} & \multicolumn{1}{r}{\tabincell{r}{DET}} & \multicolumn{1}{r}{800}\\
\hline
{\bfseries Total} & \multicolumn{1}{c}{N/A} & \multicolumn{1}{r}{N/A} & \multicolumn{1}{r}{178,757}\\
\hline
\end{tabular}
%}
\label{tab1}
%\vspace{-5mm}
\end{table}

==> pne-mura-res-tab-v1.tex <==

\begin{table}[t]
\centering
\caption{Performance Comparisons for Pneumonia Classification (Pneumonia) and Skeletal Abnormality Classification (MURA) using various Pre-training Algorithms.}\label{tab2}
\begin{tabular}{p{50pt}p{50pt}p{40pt}p{40pt}p{40pt}p{40pt}p{40pt}p{40pt}p{40pt}p{40pt}}
\hline
\multirow{2}*{\bf Backbones} & \multirow{2}*{\bf Pre-train} & \multicolumn{4}{c}{\bfseries Pneumonia} & \multicolumn{4}{c}{\bfseries MURA}\\
\cmidrule(r){3-6}  \cmidrule(r){7-10}
 & & \multicolumn{1}{c}{\bfseries Acc.} & \multicolumn{1}{c}{\bfseries AUC} & \multicolumn{1}{c}{\bfseries Sen.} & \multicolumn{1}{c}{\bfseries Spe.} & \multicolumn{1}{c}{\bfseries Acc.} & \multicolumn{1}{c}{\bfseries AUC} & \multicolumn{1}{c}{\bfseries Sen.} & \multicolumn{1}{c}{\bfseries Spe.}\\
\hline
\multirow{5}*{ResNet-18}
& Scratch & \multicolumn{1}{r}{91.11} & \multicolumn{1}{r}{96.59} & \multicolumn{1}{r}{93.91} & \multicolumn{1}{r}{83.54} & \multicolumn{1}{r}{81.00} & \multicolumn{1}{r}{86.66} & \multicolumn{1}{r}{68.17} & \multicolumn{1}{r}{\bfseries 89.91}\\
& ImageNet & \multicolumn{1}{r}{90.09} & \multicolumn{1}{r}{96.16} & \multicolumn{1}{r}{93.68} & \multicolumn{1}{r}{80.38} & \multicolumn{1}{r}{81.88} & \multicolumn{1}{r}{88.10} & \multicolumn{1}{r}{73.49} & \multicolumn{1}{r}{87.70}\\%\hline
& MD-MoCo & \multicolumn{1}{r}{96.58} & \multicolumn{1}{r}{98.49} & \multicolumn{1}{r}{97.19} & \multicolumn{1}{r}{94.94} & \multicolumn{1}{r}{82.48} & \multicolumn{1}{r}{88.29} & \multicolumn{1}{r}{72.27} & \multicolumn{1}{r}{89.57}\\
& \TheName{}$^{--}$ & \multicolumn{1}{r}{96.75} & \multicolumn{1}{r}{99.51} &  \multicolumn{1}{r}{\bfseries 97.66} &  \multicolumn{1}{r}{94.30} & \multicolumn{1}{r}{82.45} & \multicolumn{1}{r}{88.40} &  \multicolumn{1}{r}{74.16} &  \multicolumn{1}{r}{88.21}\\
& \TheName{} & \multicolumn{1}{r}{\bfseries 97.26} & \multicolumn{1}{r}{\bfseries 99.60} &  \multicolumn{1}{r}{97.42} &  \multicolumn{1}{r}{\bfseries 96.84} & \multicolumn{1}{r}{\bfseries 82.62} & \multicolumn{1}{r}{\bfseries 88.52} &  \multicolumn{1}{r}{\bfseries 74.28} &  \multicolumn{1}{r}{88.42}\\
\hline
\multirow{5}{*}{ResNet-50}
& Scratch & \multicolumn{1}{r}{91.45} & \multicolumn{1}{r}{96.58} & \multicolumn{1}{r}{92.51} & \multicolumn{1}{r}{88.61} & \multicolumn{1}{r}{80.50} & \multicolumn{1}{r}{86.24} & \multicolumn{1}{r}{65.42} & \multicolumn{1}{r}{90.97}\\
& ImageNet & \multicolumn{1}{r}{95.38} & \multicolumn{1}{r}{98.75} & \multicolumn{1}{r}{95.78} & \multicolumn{1}{r}{94.30} & \multicolumn{1}{r}{81.73} & \multicolumn{1}{r}{87.92} & \multicolumn{1}{r}{68.36} & \multicolumn{1}{r}{\bfseries 91.01}\\%\hline
& MD-MoCo & \multicolumn{1}{r}{97.09} & \multicolumn{1}{r}{99.52} & \multicolumn{1}{r}{\bfseries 98.83} & \multicolumn{1}{r}{92.41} & \multicolumn{1}{r}{82.35} & \multicolumn{1}{r}{87.95} & \multicolumn{1}{r}{73.12} & \multicolumn{1}{r}{88.76}\\
& \TheName{}$^{--}$ & \multicolumn{1}{r}{96.75} & \multicolumn{1}{r}{99.58} & \multicolumn{1}{r}{98.36} & \multicolumn{1}{r}{92.41} & \multicolumn{1}{r}{81.10} & \multicolumn{1}{r}{87.15} & \multicolumn{1}{r}{69.03} & \multicolumn{1}{r}{89.48}\\
& \TheName{} & \multicolumn{1}{r}{\bfseries 98.12} & \multicolumn{1}{r}{\bfseries 99.72} & \multicolumn{1}{r}{98.36} & \multicolumn{1}{r}{\bfseries 97.47} & \multicolumn{1}{r}{\bfseries 82.60} & \multicolumn{1}{r}{\bfseries 88.41} & \multicolumn{1}{r}{\bfseries 74.53} & \multicolumn{1}{r}{88.21}\\
\hline
\end{tabular}
%\vspace{-5mm}
\end{table}

